Timed Automata Semantics for Analyzing Creol

We give a real-time semantics for the concurrent, object-oriented modeling language Creol, by mapping Creol processes to a network of timed automata. We can use our semantics to verify real time properties of Creol objects, in particular to see whether processes can be scheduled correctly and meet their end-to-end deadlines. Real-time Creol can be useful for analyzing, for instance, abstract models of multi-core embedded systems. We show how analysis can be done in Uppaal.

==> eptcsdata.tex <==
\providecommand{\firstpage}{108}
\providecommand{\publicationstatus}{M.R. Mousavi and G. Sala{\"u}n (Ed.): International
Workshop \\ on the  Foundations of Coordination Languages and \\ Software Architectures (FOCLASA 2010).\\
EPTCS 30, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.30.8}{10.4204/EPTCS.30.8}}
\pdfoutput=1

